Instant-NeRF: Instant On-Device Neural Radiance Field Training via Algorithm-Accelerator Co-Designed Near-Memory Processing

Instant on-device Neural Radiance Fields (NeRFs) are in growing demand for unleashing the promise of immersive AR/VR experiences, but are still limited by their prohibitive training time. Our profiling analysis reveals a memory-bound inefficiency in NeRF training. To tackle this inefficiency, near-memory processing (NMP) promises to be an effective solution, but also faces challenges due to the unique workloads of NeRFs, including the random hash table lookup, random point processing sequence, and heterogeneous bottleneck steps. Therefore, we propose the first NMP framework, Instant-NeRF, dedicated to enabling instant on-device NeRF training. Experiments on eight datasets consistently validate the effectiveness of Instant-NeRF.

==> sections/backup.tex <==
In particular, we utilize Morton encoding~\cite{z-order} (also known as Z-order) to formulate the following hashing function from the vertex location ($\mathbf{x}\in\mathbb{Z}^3$) to the hash table entry index ($f(\mathbf{x})\in\mathbb{Z}$):
\begin{align}
f(\mathbf{x})=\left(x^{\prime}_{0} \oplus (x^{\prime}_{1} \ll 1) \oplus (x^{\prime}_{2} \ll 2) \right) \quad \bmod T \label{eq:zorder_hash}
\end{align}
where $T$ is the number of hash table entries; \(\oplus\) denotes the bit-wise \(\mathrm{XOR}\) operation; and $x^{\prime}$ is the 32 bits binary format of each dimension through Eq.~(\ref{eq:bit_expand}).
\begin{align}
x^{\prime}= (((x * p_{1}) \land  q_{1})* p_{2}) \land q_{2})   \label{eq:bit_expand}
\end{align}
here, the binary format output $x^{\prime}$=$x^{\prime}_{4}$ and initial input is $x^{\prime}_{0}$=$x$. $p$ $q$ are hyper parameters, with $p=\{$0x00010001, 0x00000101, 0x00000011, 0x00000005\} and $q=\{$0xFF0000FF, 0x0F00F00F, 0xC30C30C3, 0x49249249\}.\y{Wrong? Simplify the description?}

% Intra-bank
\textbf{Intra-Bank Dataflow.} an optimal inter-bank parallelism should balance the 

\textbf{Data Layout Between Traditional Address Mapping and {\name}'s Address Mapping.} 
A context MUX is placed before the bank address decoder (i.e., Row Dec. and Column Dec. in Fig.~\ref{fig:hw_overall}(c)) which is controlled the host processor. Once the {\name} is enabled by the host processor. In order to exploit bank-level memory bandwidth, we integrate the {\name} logic near every memory bank (Fig.~\ref{fig:hw_overall}(d)). To switch between a normal memory bank and an {\name} accelerator, a context MUX is placed before the bank address decoder (i.e., Row Dec. and Column Dec. in Fig.~\ref{fig:hw_overall}(c)) which is controlled the host processor. Once the {\name} is enabled by the host processor, 

Besides the intrinsic bank-level parallelism at each memory bank, i

The command and address generators take the row addresses from the row-address FIFO  initiate LPDDR4 C/A signals which are sent to the memory bank. Compared to standard C/A signals, we add a new subarray ID signal and do not deploy unnecessary features like \todor{XX (ask Jingqun)}. 
% =======================

since the input data in HT is duplicated which is only 12\% of the multiresolution hash table size, while the MLP weight is duplicated in MLP which is 1\% of the input data in MLP. 

We analyze the computation and memory patterns of the heterogeneous bottleneck steps involving hash table lookup and MLP processing. Based on the analysis, we propose dedicated inter-bank and intra-bank designs for these steps.

Besides the parameter/data duplication, Fig.~\ref{fig:inter-bank} also demonstrates the other three operations incurring inter-bank data movements: the input/output data transfer between steps/kernels, the intermediate data transfer in one step/kernel, and the gradient partial sum summation (\ding{173}, \ding{174}, and \ding{175} in Fig.~\ref{fig:inter-bank}). Thanks 

Tab.~\ref{tab:data_size} illustrates the parameter and data sizes for the bottleneck steps/kernels in NeRF trainig. Following the aforementioned principle, we elaborate parameter parallelism and data parallelism for HT/HT\_b and MLP/MLP\_b, respectively, as in Fig.~\ref{fig:inter-bank}. 

Our proposed heterogeneous inter-bank parallelism designs can achieve a minimum total inter-bank 

The heterogeneous steps involving hash table lookup and MLP processing, exhibit different data size patterns as illustrated in Tab.~\ref{tab:data_size}. 

To minimize inter-bank data movements, we can summarize the following \textbf{Inter-bank parallelism principle:} data parallelism favors steps/kernels with a smaller parameter size, while parameter parallelism benefits steps/kernels a smaller input data size.

There are two methods to  to distribute computations among multiple banks (e.g., 16 physical banks in LPDDR4~\cite{oh20143lpddr4}) to explore the benefits of inter-bank parallelism. 

Tab.~\ref{tab:data_size} illustrates the parameter/data sizes for the 4 steps/kernels. As limited by the I/O interface and the internal prefetch width (see Fig.~\ref{fig:lpddr}), the memory latency to access data in other banks is much higher than that in the local bank. 

\textbf{Overview.} As shown in Fig.~\ref{fig:hw_overall}(a), the {\name} architecture is deployed at one or several DRAM dies. In order to exploit bank-level memory bandwidth, we integrate the {\name} logic near every memory bank and call a memory die with {\name} logic as an {\name} accelerator. Each memory bank supports subarray parallelism through integrating individual subarray row-address latches for the subarrays~\cite{kim2012case}, as illustrated in Fig.~\ref{fig:hw_overall}(c). 

We introduce the overall organization and opportunities of Low Power Multiple Dual In Memory Module 4 (LPDDR4)~\cite{lpddr4x}, a DRAM type which is widely used by edge devices~\cite{tx2,xnx}, for NeRF training as follows. As shown in Fig.~\ref{fig:lpddr}, an LPDDR4 channel typically has 1 rank with 1 die/rank. An LPDDR4 die consists of 16 physical banks, which share a common I/O interface and internal I/O buffers. While the I/O interface width is 16b and the internal prefetch structure has a width of 256b (i.e., 16n prefetch structure), the row buffer within each bank provides a data width of 1KB. This row buffer organization provides intrinsic parallelism~\cite{devic2022pim} which can be leveraged to address the \textbf{memory bandwidth} bottleneck for NeRF training. In addition, for a typically adopted 8/16GB 128bit LPDDR4 memory system in edge devices~\cite{tx2,xnx}, each bank has 128$\sim$256MB capacity, providing enough \textbf{memory capacity} for steps in NeRF training. Furthermore, as a bank is further composed of subarrays (Fig.~\ref{fig:hw_overall}(c)), subarray parallelism has been explored by prior works~\cite{kim2012case} to deal with the \textbf{bank conflict} challenge, which is discussed in Sec.~\ref{sec:intro}. 

Since NeRF training's bottleneck steps/kernels contain heterogeneous data types, i.e., INT32 and FP32, both INT32 and FP32 arithmetic should be efficiently supported by the computation engine. In addition, as these steps/kernels involve vector and matrix computations (e.g., trilinear interpolation and MLPs), it is natural for {\name} logic to include vector processing engines (PEs) to optimize for the repeated operations across vector/matrix~\cite{devic2022pim} 

two row-buffer sized vector processing elements (PEs), 3 row-buffer sized vector registers for vector PEs (v1, v2, and v3), a crossbar for data transfer between  

Since NeRF training's bottleneck steps/kernels contain heterogeneous data types, i.e., INT32 and FP32, both INT32 and FP32 arithmetic should be efficiently supported. In addition, as these steps/kernels involve vector and matrix computations (e.g., trilinear interpolation and MLPs), it is natural for {\name} logic to include vector processing engines (PEs) to optimize for the repeated operations across vector/matrix~\cite{devic2022pim}. Therefore, 

the computation resource within each {\name} 

Specifically, our {\name} logic has two row-buffer sized vector processing engine (PEs) for FP32 and INT32 arithmetic as shown in , respectively.


Since NeRF training's bottleneck steps/kernels involve vector and matrix computations (e.g., trilinear interpolation and MLPs), {\name} logic should include vector processing engines (PEs) to optimize for the repeated operations across vector/matrix elements. In addition, as heterogeneous data types, i.e., INT32 and FP32, are utilized, both INT32 and FP32 arithmetic should be supported. Therefore, we add two row-buffer sized vector PEs for INT32 and FP32 arithmetic

,  for FP32 and INT32 arithmetic, respectively.

we add both INT32 and FP32 arithmetic to {\name} logic. Specifically, as shown in Fig.~\ref{fig:hw_overall}(d), we add two row-buffer sized vector processing engine (PEs) for FP32 and INT32 arithmetic, respectively.

Neural Radiance Field (NeRF) enabled on-device 3D reconstruction suffers from long training time, which prevents its practical deployment on Augmented/Virtual Reality devices. Our profiling on state-of-the-art edge devices unveils the memory-bound bottleneck for NeRF training. Therefore, this work proposes the first Near-Memory Processing (NMP) framework, {\name}, for instant NeRF training utilizing a near-bank architecture with subarray parallelism. 
Algorithm-level innovations including locality-sensitive hashing function and NMP-friendly point stream order are proposed. Hardware-level innovations including an optimal mapping scheme and supports for heterogeneous bottlenecks steps are proposed, achieving \todor{XX}$\times$ speedup over baselines without sacrificing the reconstruction quality. 

GPU schedules for grouping the write operations to the same gradient and cannot achieve ideal performance. 

\textbf{Opportunity of NMP-based NeRF Training.} Offloading the memory-bound bottleneck steps to NMP architecture is a promising solution to boost NeRF training efficiency. Near-bank NMP architecture benefits from the 10$\times$ peak bandwidth improvement to solve the memory bandwidth bottleneck. In addition, the hundreds of MB memory per bank (i.e,. 256MB in our evaluation) provides enough memory capacity for steps in NeRF training. 

\textbf{Challenge of NMP-based NeRF Training.} However, even if providing enough memory capacity, naive NMP architectures cannot efficiently support NeRF training due to three challenges. \textbf{First}, random hash table lookup can potentially cause a reduced effective memory bandwidth for NMP architecture, because memory requests are at the granularity of a memory bank row buffer (e.g., 1~2KB~\cite{devic2022pim, lpddr4x}) while each hash table feature vector is only 32-bit. Furthermore, random hash table lookup can potentially cause bank conflicts if two memory requests go the same bank but different addresses. Bank conflicts, consequently, serialize computations that can be served in parallel, harming the performance. \textbf{Second}, the random processing sequence of points can lead to non-sequential accesses to same hash table feature vector values/gradients in Hashtable and Hashtable\_b kernels, respectively. As a result, hash table lookup that could have otherwise hit in local registers of the computation logic will miss in local registers, incurring long-latency memory requests to memory banks. \textbf{Third}, heterogeneous bottleneck steps involving hashing, hash table lookup, and MLP processing exhibit various data types (i.e., INT32, FP32) and computation and memory patterns, thus requiring dedicated support. Algorithm- and hardware-level innovations are proposed in {\name} to solve these challenges. 

\begin{table*}[tbp]
\caption{Evaluated platforms \textcolor{red}{Chaojian give the sparsity of the matrix of the 8 datasets}}
\centering
% \vspace{-1em}
  \resizebox{\linewidth}{!}
  {
 % V100 3970 Cloud TX2 4b ICARUS edge
    \begin{tabular}{c||ccc||cccc}
    \toprule
    \multirow{2}{*}{\textbf{Chip}}& \multicolumn{3}{c||}{\textbf{Cloud Servers}} & \multicolumn{4}{c}{\textbf{Edge Devices}} \\
    & \textbf{NVIDIA V100} & \textbf{AMD Ryzen 3970x} & \textbf{RT-NeRF-Cloud} & \textbf{NVIDIA Tegra X2} & \textbf{Raspberry Pi 4 Model B} & \textbf{ICARUS} &  \textbf{RT-NeRF-Edge} \\
    \midrule
    Computing & 80 (SM) & 32 (Core) & 30 (Core) & 2 (SM) & 4 (Core) & N/A & 1 (Core) \\
    Units      & 5120 (CUDA) & 64 (Thread) & 30 (SPU) + 90 (PPU) & 256 (CUDA) & 4 (Thread) & N/A & 1 (SPU) + 3 (PPU) \\
    \midrule
    SRAM & 36 MB & 146MB & 105 MB & 2.6 MB & 1.32MB & 0.96MB& 3.5 MB \\
    \midrule
    Area (mm$^2$)& 815 & 296 & 250.5 & 350 & 100 & N/A & 8.35 \\
    \midrule
    Frequency & 1.5 GHz & 3.7GHz & 1 GHz & 1.3 GHz & 1.5GHz & 0.3GHz& 1 GHz \\
    \midrule
    DRAM & HBM2 & DDR4-3200 & DDR4-3200 & LPDDR4-1866 & LPDDR4-2400 & N/A & LPDDR4-2400\\
    Bandwidth & 900 GB/s & \textcolor{red}{chaojian} & 14.4 GB/s & 59.7 GB/s & \textcolor{red}{chaojian} & N/A & 0.48 GB/s\\
    \midrule
    Technology & 12 nm & 7nm & 28 nm & 16 nm & 28nm & 40nm & 28 nm \\
    \midrule
    % Peak Performance & 15.7 TOPS & 864 GOPS & 1.3 TOPS & 144 GOPS \\
    % \midrule
    Typical Power & 300 W & 270 W & 240 W & 15 W & 6 W & 0.3 W & 8 W \\
    \midrule
    Typical FPS & 200 & \textcolor{red}{chaojian} & 1800 & 4 & \textcolor{red}{chaojian} & 0.029 & 60 \\
    \bottomrule
    % Full load 36, 30% sparsity 120
    \end{tabular}
    }
  \label{tab:platform}
\end{table*}



We show in Fig.~\ref{fig:iNGP_kernel}(a) that over \todob{X}\% of the operations are...

\todob{Profiling on XNX can be generalized to other SOTA edge devices for AR/VR.}

% Although emerging Near-Memory Processing (NMP) technologies~\cite{yitbarek2016exploring, kwon2019tensordimm, asgari2021fafnir} have the potential to accelerate NeRF training through addressing the memory-bound problem, there are still several challenges. 

Challenges: 
Limited locality --> accesses local random accesses and remote random access;
Access granularity


In particular, we locate three efficiency-bottleneck steps (see Fig.~\ref{fig:iNGP_alg}): \textbf{Step}~{\color{black}{\ding{184}}} accessing the multiresolution hash table and the following linear interpolations; \textbf{Step} {\color{black}{\ding{188}}} processing the backward step of \textbf{Step}~{\color{black}{\ding{184}}}; and \textbf{Step} {\color{black}{\ding{185}}} computing the features (i.e., densities and colors) of the points through MLPs. 
Furthermore, we find that \textbf{Step}~{\color{black}{\ding{184}}} and \textbf{Step}~{\color{black}{\ding{185}}} show apparent bandwidth-bound performance bottleneck, since \todor{X}\%/\todor{X}\% DRAM bandwidth utilization v.s. \todor{X}\%/\todor{X}\% ALU utilization for \textbf{Step}~{\color{black}{\ding{184}}}/\textbf{Step}~{\color{black}{\ding{185}}} (see Fig.~\ref{fig:iNGP_kernel}(a)) consuming 45.9\% of the overall training time (see Fig.~\ref{fig:iNGP_comp}(b)). 
The underlying reason is that the limited L2 cache (i.e., 256KB)~\cite{xnx} is too small for individual levels of the hash table in the algorithm (i.e., 2MB)~\cite{muller2022instant} for \textbf{Step}~{\color{black}{\ding{184}}} and the intermediate data for \textbf{Step}~{\color{black}{\ding{185}}}, resulting in massive DRAM accesses.
In addition, we find that the remaining dominant \textbf{Step}~{\color{black}{\ding{188}}} (accounting for 30.5\% of training time) shows low utilization for both memory and ALU, which results from that the step involves value-dependent computations and GPU cannot achieve ideal performance due to the limited parallelism.


\todob{TODO: 1) Consistency with Fig.~\ref{fig:iNGP_Pipeline}. 2) Cube (8*vertices), Vertices' location --> hash --> index, Lookup feature vector array.}
The training pipeline of iNGP is similar to other voxel based neural rendering method but replaces an explicit grid structure with a multi-resolution hash encoding and can be summaized as follow: \ding{172} \textbf{Voxels collection}: Finds a set of voxels at different resolution levels through a spatial hash function~\cite{muller2003optimized} based on one given input coordinate \textbf{x} \todob{No need to show this hash function?}. The hash function is:
\begin{align}
h(\mathbf{x})=\left(\bigoplus_{i=1}^{d} x_{i} \pi_{i}\right) \quad \bmod T,
\end{align}
where \(\oplus\) denotes the bit-wise \(\mathrm{XOR}\) operation, \(\pi_{i}\) are unique, large prime numbers and T is the hash table size for each level~\cite{muller2022instant}.\ding{173} \textbf{Fetch features}: After collecting nearby voxels, it will fetch corresponding feature vectors from hash table and \ding{174} \textbf{Interpolation}: Apply linear interpolation to get the feature vectors of input coordinate \textbf{x}. \ding{175} \textbf{Density MLP Forward}: Then it will concatenate across all levels and gives into density MLP model. \ding{176} \textbf{Color MLP Forward}: The output of the density MLP model will be encoded with view direction information and then gives into the color MLP model.


Neural Radiance Field (NeRF) enabled on-device 3D reconstruction suffers from long training time, which prevents its practical deployment on Augmented/Virtual Reality (AR/VR) devices. Our profiling on state-of-the-art (SOTA) edge devices unveils the memory bandwidth and capacity bottlenecks for NeRF training. As such, this work proposes the first Near-Memory Processing (NMP) accelerator, {\name}, for instant NeRF training utilizing a near-bank architecture with sub-array parallelism. 
An optimal hash table mapping scheme, an NMP-friendly sampling points grouping algorithm, and dedicated inter-bank parallelisms are integrated into {\name} to address the random hash table access, random processing sequence of sampling points, and heterogeneous bottleneck steps challenges, respectively. 
{\name} achieves \todor{XX}$\times$ speedup over baselines while maintaining the same reconstruction quality. 

Recently, Neural Radiance Field (NeRF) has yielded state-of-the-art (SOTA) performance for reconstructing 3D scenes from a set of sparsely sampled views, enabling various applications in Augmented and Virtual Reality (AR/VR). However, NeRF-based on-device 3D reconstruction suffers from long training time since the efficiency-bottleneck steps require a high memory bandwidth and a large memory footprint, way exceed the AR/VR device capacity. 
This work proposes the first Near-Memory Processing (NMP) accelerator {\name} for NeRF training using near-bank architecture with sub-array parallelism. 
{\name} achieves average \todor{X}$\times$ sppedup 
To tackle the random 
{\name} achieves average \todor{X}$\times$ speedup without accuracy loss compared with SOTA 

Specifically, iNGP represents the 3D scene with a multiresolution hash table followed by two small multi-layer perception networks (MLPs) for density and RGB color features, respectively. 

\textbf{Step}~{\color{black}{\ding{184}}} even the individual levels of the hash are stored and processed near-bank; and naive NMP architectures lack the optimization for the value-dependent \textbf{Step}~{\color{black}{\ding{185}}}. 

Furthermore, we identify the underlying reason for these steps' bottleneck inefficiency is that these steps require a high memory bandwidth and a large memory footprint than the memory subsystem on the edge device can provide.


since they have low arithmetic intensity 

have low arithmetic intensity but demands high memory bandwidth and 


accessing the vertices around the points in the multiresolution hash table and followed by 
which includes accessing the multiresolution hash table and 
accessing the multiresolution hash table and calculating the following trilinear interpolations; (2) 

We follow a two-step profiling: (1) characterizing the runtime of each step in the algorithm pipeline to locate the dominate steps and (2) profiling the DRAM bandwidth utilization and ALU utilization of the dominant steps (and their corresponding backward steps). 
In particular, we locate three efficiency-bottleneck steps (see Fig.~\ref{fig:iNGP_alg}): \textbf{Step}~{\color{black}{\ding{184}}} accessing the multiresolution hash table and the following linear interpolations; \textbf{Step} {\color{black}{\ding{188}}} processing the backward step of \textbf{Step}~{\color{black}{\ding{184}}}; and \textbf{Step} {\color{black}{\ding{185}}} computing the features (i.e., densities and colors) of the points through MLPs. 
Furthermore, we find that \textbf{Step}~{\color{black}{\ding{184}}} and \textbf{Step}~{\color{black}{\ding{185}}} show apparent bandwidth-bound performance bottleneck, since \todor{X}\%/\todor{X}\% DRAM bandwidth utilization v.s. \todor{X}\%/\todor{X}\% ALU utilization for \textbf{Step}~{\color{black}{\ding{184}}}/\textbf{Step}~{\color{black}{\ding{185}}} (see Fig.~\ref{fig:iNGP_kernel}(a)) consuming 45.9\% of the overall training time (see Fig.~\ref{fig:iNGP_comp}(b)). 
The underlying reason is that the limited L2 cache (i.e., 256KB)~\cite{xnx} is too small for individual levels of the hash table in the algorithm (i.e., 2MB)~\cite{muller2022instant} for \textbf{Step}~{\color{black}{\ding{184}}} and the intermediate data for \textbf{Step}~{\color{black}{\ding{185}}}, resulting in massive DRAM accesses.
In addition, we find that the remaining dominant \textbf{Step}~{\color{black}{\ding{188}}} (accounting for 30.5\% of training time) shows low utilization for both memory and ALU, which results from that the step involves value-dependent computations and GPU cannot achieve ideal performance due to the limited parallelism.

even if the individual levels of the hash table are stored and processed near-bank

To overcome the bottleneck of memory bandwidth, the Near-Memory Processing (NMP) architecture~\cite{yitbarek2016exploring, kwon2019tensordimm, asgari2021fafnir} introduces a promising solution. This architecture embraces higher memory bandwidth by integrating compute-logic nearer to memory. Take DIMM as an example, recent works deploy the compute-logic at rank-, bank-, or even subarray-level~\cite{asgari2021fafnir} to enjoy the \todor{X$\sim$X}$\times$ peak bandwidth improvement. 
However, naive NMP architectures cannot efficiently support the random hash table read accesses involved by \textbf{Step}~{\color{black}{\ding{184}}} even the individual levels of the hash are stored and processed near-bank; and naive NMP architectures lack the optimization for the value-dependent \textbf{Step}~{\color{black}{\ding{185}}}. 
let alone the massive data write accesses for storing the data for backward processing (i.e., ) in \textbf{Step}~{\color{black}{\ding{184}}}




First, the random hash table accesses can potentially cause a reduced effective memory bandwidth since memory accesses are at the granularity of a memory row (e.g., 1KB~\cite{devic2022pim}) while each hash table entry is only 16-bit. Furthermore, random hash table accesses can potentially cause bank conflicts if two memory access requests go the the same bank but different addresses. Bank conflicts, consequently, serialize computations that can be served in parallel.
Second, 

Second, the random processing sequence of points can lead to non-sequential accesses to the same hash table entries and thus  


64 values in the hash table. which can contain unused hash table values since each hash table value is only 16b. 
(1) The first challenge is the random hash table access. Random hash table accesses can potentially cause a reduced effective memory throughput because data are read/write from/to memory banks at the granularity of a memory row (e.g., 1KB~\cite{devic2022pim}) while each hash table entry is only 16-bit. Furthermore, random hash table accesses can potentially cause bank conflicts if two memory requests go the the same bank but different addresses. Bank conflicts, consequently, serialize computations that can be served in parallel.
(1) a reduced effective memory throughput since the data are read/write from/to memory banks at the granularity of memory rows, which can usually contains 64 values in the hash table.

and (2) bank conflicts if two memory access requests go the the same bank but different addresses thus serialize computations that can be served in parallel. 

ranularity for each read/write access .
Second, the heterogeneous bottleneck steps involving hash table accessing and MLP processing exhibit various computation and memory patterns, thus requiring dedicated hardware support for each step.   

    The key component of {\name} is a tree structure (Sec.~\ref{}), the leaves of which are the banks in a memory chip and the chunk nodes of which are integrated with content addressable memory (CAM) to cache memory accesses for non-local banks. The tree structure provides two-folds of benefits: (1) The amount of hash table read accesses to non-local banks is reduced by merging the accesses to the same addresses; and (2) the value-dependent step is decoupled into a reduction of parallel value-dependent sub steps with improved parallelism. 
    

Our {\name} takes advantages of the near-bank NMP architecture with subarray-parallelism and tackles the new challenges in NeRF training throughput an algorithm-hardware co-design approach. 
Near-Memory processing techniques are widely used to solve the memory-bound problems, thanks to the larger internal bandwidth provided.
In particular, many neural network workloads are memory intensive, thus prior studies~\cite{yitbarek2016exploring, shin2018mcdram} exploit NMP architectures for Neural Network (NN) workloads.  
The bank conflict latencies can be dramatically reduced by exploring the sub0array-level parallelism~\cite{kim2012case}. 

==> sections/backup_1-Introduction.tex <==
\section{Introduction}
\label{sec:intro}

Modeling and reconstructing 3D scenes from a set of sparsely sampled views is crucial for various applications in Augmented and Virtual Reality (AR/VR), such as virtual meetings~\cite{workrooms}. Recently, Neural Radiance Field (NeRF) and its many follow-up works~\cite{mildenhall2020nerf, sun2021direct, muller2022instant} have shown success on modeling a scene as a neural radiance field and yielded state-of-the-art (SOTA) rendering quality. Many works have demonstrated significant speedup of NeRF-based rendering~\cite{iccad_2022} and NeRF-based 3D reconstruction on cloud GPUs~\cite{sun2021direct, muller2022instant}. However, NeRF-based 3D reconstruction on edge devices, i.e., edge GPUs as SOTA accelerators for AR/VR devices~\cite{quest_pro}, is still impeded by the need of lengthy training time. This makes NeRF infeasible for many application scenarios~\cite{sun2021direct}. 
Fig.~\ref{fig:iNGP_comp}(a) shows that when running the SOTA NeRF training method on one SOTA edge GPU, about two hours of per scene training is required, resulting in a 23$\times$ longer training time than that on a cloud GPU. 
% Fig.~\ref{fig:iNGP_comp}(a) shows that when running the SOTA training method (i.e., iNGP~\cite{muller2022instant}) on an edge GPU (i.e., XNX~\cite{xnx}), about two hours of per scene training is required, resulting in a 23$\times$ longer training time than that on a cloud GPU (i.e., 2080Ti~\cite{2080ti}). 

%%%%%%%%%%%%%% Begin of Figure %%%%%%%%%%%% 
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/fig1_server_edge.pdf}
  \vspace{-2.5em}
  \caption{An comparison of training time when running the SOTA efficient NeRF training method, i.e.,  iNGP~\cite{muller2022instant}, on a cloud GPU (i.e., 2080Ti~\cite{2080ti}) and an edge GPU (i.e., XNX~\cite{xnx}).}
  \vspace{-1.5em}
  \label{fig:iNGP_comp}
\end{figure}
%%%%%%%%%%%%%%  End of Figure  %%%%%%%%%%%%

To close the aforementioned training efficiency gap on edge devices, we first perform in-depth profiling of the SOTA efficient NeRF training method, i.e., iNGP~\cite{muller2022instant}, on the edge GPU, i.e., XNX~\cite{xnx}, to identify the bottlenecks. 
Specifically, iNGP represents the 3D scene with a multiresolution hash table of trainable location feature vectors followed by two small multi-layer perception networks (MLPs) for density and RGB color features, respectively. Our profiling results reveal three efficiency-bottleneck steps in the SOTA training method (see Fig.~\ref{fig:iNGP_comp}(b)): (1) computing points' encoding features by trilinearly interpolating the corresponding surrounding 3D cubes' 8 vertices of features of  multi-level grids; (2) back-propagation of multi-level grids' features; and (3) calculating point's density and RGB color features through MLPs (and their back-propagations).
Furthermore, we find that these three steps show apparent DRAM bandwidth-bound performance bottleneck, where the measured memory bandwidth utilization is 5.24$\sim$21.44$\times$ higher than FPU/ALU utilization. The underlying reasons for this memory-bound inefficiency are that (1) random accesses to the hash table, which stores multi-level grids' features, require a high memory bandwidth and (2) the cache capacity is too small for individual levels of the hash table and intermediate data when processing MLPs.

To overcome the memory-bound inefficiency bottleneck, emerging Near-Memory Processing (NMP) architecture~\cite{devic2022pim, kwon2019tensordimm, asgari2021fafnir} introduces a promising solution. This architecture embraces higher memory bandwidth by integrating computation logic nearer to memory. For example, recent works deploy the computation logic at bank-level in DIMM to enjoy around 10$\times$ peak bandwidth improvement~\cite{devic2022pim}. 

However, even if providing enough memory capacity, naive NMP architectures cannot efficiently support NeRF training due to three challenges. 
First, random hash table accesses, when calculating each individual point, can potentially cause a reduced effective memory bandwidth because memory requests are at the granularity of a memory row (e.g., 1KB~\cite{devic2022pim}) while each hash table entry is only 16-bit. Furthermore, random hash table accesses can potentially cause bank conflicts if two memory requests go the same bank but different addresses. Bank conflicts, consequently, serialize computations that can be served in parallel.
Second, the random processing sequence of points can lead to non-sequential accesses to same hash table entries. As a result, hash table accesses that could have otherwise hit in local registers of the computation logic will miss in local registers, incurring long-latency memory requests to memory banks. 
Third, heterogeneous bottleneck steps involving hash table accessing and MLP processing exhibit various computation and memory patterns, thus requiring dedicated support for each step.

Therefore, we propose the first NMP solution, dubbed as {\name}, to address the identified memory-bound problem to boost on-device NeRF training efficiency. 
To overcome the first challenge, we develop a hash table mapping scheme based on the analysis of the hash table keys of surrounding 3D cubes' 8 vertices. Specifically, the mapping scheme maps vertices along unpermuted dimension on the same memory rows to increase effective memory bandwidth. In addition, the mapping scheme distributes the vertices along the other two dimensions to different subarrays to reduce bank conflicts. The mapping scheme further enables locality-sensitive vertex encoding and inter-level mapping to schedule the vertices from different resolution levels but within the same regions of the scene on the same memory rows to increase effective memory bandwidth.
To address the second challenges, a NMP-friendly grouping algorithm is proposed based on the fact that points having same surrounding 3D cubes will access same hash table entries. The grouped points are then streamed to {\name} sequentially to increase local register hit rates and reduce unnecessary memory requests. Please note that {\name} accelerates the grouping algorithm as well, resulting in negligible overhead (i.e., \todor{X\%} of processing time).  
The third challenge related to heterogeneous bottleneck steps is tackled by designing dedicated inter-bank parallelism schemes for each step. In particular, steps involving hash table accessing utilize multiresolution hash table inter-bank parallelism and duplicate data among banks; while steps involving MLP processing utilize data inter-bank parallelism and duplicate MLP parameters among banks.  

The contributions of our contributions are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item We study the SOTA efficient NeRF training method~\cite{muller2022instant} on SOTA commercial edge devices over 8 datasets and identify the memory-bound performance bottleneck steps, which are the primary causes of SOTA training method's inefficiencies (Sec.~\ref{sec:motivation}).
    \item We propose a DIMM-based NMP accelerator {\name} using near-bank architecture with subarray parallelism, which to the best of our knowledge, is the first NMP solution for achieving instant on-device NeRF training. 
    \item For {\name}, we develop a hash table mapping scheme (Sec.~\ref{mapping}) to tackle the challenge of random hash table accesses; we propose a grouping algorithm with NMP support (Sec.~\ref{grouping}) to group the points with same hash table entries together and then process the grouped points sequentially to increase local register hit rates; and we enable dedicated inter-bank parallelisms (Sec.~\ref{ISA}) to support heterogeneous bottleneck steps. 
    \item We build a cycle-accurate simulator extended from Ramulator~\cite{kim2015ramulator} to evaluate the performance of {\name}. Comprehensive experiments show that {\name} provides \todor{XX$\times$} average speedup over the edge GPU baseline while maintaining a similar rendering quality. 
    
\end{itemize}

We introduce the preliminary background and related works in Sec.~\ref{sec:background} and discuss our evaluation methodology and experimental results in Sec.~\ref{sec:evaluation}. 



==> sections/backup_3-Motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\subsection{Profiling SOTA Efficient NeRF Training Method on SOTA GPUs}

%%%%%%%%%%%%%%  Begin of Table  %%%%%%%%%%%%
\begin{table}[t]
\caption{A summary of the considered SOTA GPUs' specs.} 
\begin{threeparttable}
\vspace{-1.3em}
\centering
%  \vspace{-1em}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c c c|c}
    \hline
    \multirow{2}{*}{\textbf{Spec.}}& \multicolumn{3}{c|}{\textbf{Edge GPUs}} & \textbf{Cloud GPU} \\
    & \textbf{XNX~\cite{xnx}} & \textbf{TX2~\cite{tx2}} & \textbf{Quest Pro$^*$~\cite{quest_pro}} & \textbf{2080Ti~\cite{2080ti}} \\ \hline
    \textbf{Tech.} & 16nm & 16nm & 7nm & \todor{TODO} \\ \hline
    \textbf{Power} & 20W\todor{?}  & 15W\todor{?}  & 5W & \todor{TODO} \\ \hline
    \multirow{3}{*}{\textbf{DRAM}}  & 128b 16GB & 128b 8GB & 64b 12GB & \todor{TODO} \\ 
                           & LPDDR4$\times$   & LPDDR4   & LPDDR5   & \todor{TODO} \\ 
                           & 59.7GB/s & 25.6GB/s & 44.0GB/s  & \todor{TODO} \\ \hline
    \textbf{GPU L2 Cache} & 512KB & 512KB & 1MB & 4MB \\ \hline
    \textbf{FP32/INT32} & 885 GFLOPS  & 750 GFLOPS  & 955 GFLOPS  & \todor{TODO} \\ \hline
    \textbf{FP16}       & 1.69 TFLOPS & 1.50 TFLOPS & 1.85 TFLOPS & \todor{TODO} \\ \hline
    \textbf{Training Time} & 7088s/scene & \todor{TODO} & N/A  & 306s/scene \\ 
    \hline
\end{tabular}
}
\end{threeparttable}
\begin{tablenotes}
\footnotesize
\item{$^*$: Specs. of Qualcomm Adreno 650 GPU, since it is used by Meta's Quest Pro~\cite{quest_pro}.}
\end{tablenotes}
\label{tab:GPU_sepc}
% \vspace{-1em}
\end{table} 
%%%%%%%%%%%%%%  End of Table    %%%%%%%%%%%%


%%%%%%%%%%%%%% Begin of Figure %%%%%%%%%%%% 
\begin{figure}[t]
  \centering
  \includegraphics[width=0.88\linewidth]{figures/fig2_kernel_profiling.pdf}
  \vspace{-1.9em}
%   \caption{(a) DRAM bandwidth, DRAM utilization, and ALU (both FP16 and INT32) utilization and (b) roofline analysis of the dominate operations (and their corresponding backward operations) when running Instant NGP~\cite{muller2022instant} training method on the edge GPU~\cite{xnx}.}
    \caption{DRAM read/write throughput and ALU (i.e., FP32, FP16, and INT32) utilization of the efficient-dominant steps/kernels (and their corresponding backward operations) when running iNGP~\cite{muller2022instant} training method on the edge GPU~\cite{xnx}.}
    \label{fig:iNGP_kernel}
\end{figure}
%%%%%%%%%%%%%%  End of Figure  %%%%%%%%%%%%

\textbf{Profiling Setup.}
\ul{Profiling Platform:} Profiling experiments have been done using SOTA GPUs including two edge GPUs (i.e., XNX~\cite{xnx} and TX2~\cite{tx2}) and one cloud GPU (i.e., 2080Ti~\cite{2080ti}). Tab.~\ref{tab:GPU_sepc} summarizes the device specifications of the selected GPUs as well as one SOTA edge GPU adopted by Meta's latest VR glass Quest Pro~\cite{quest_pro}. Since the edge GPUs used for profiling (especially XNX) have comparable on-chip cache and peak computation performance (i.e., FP32/16 and INT32 performance) and even higher DRAM bandwidth than the edge GPU adopted by the latest VR/AR device, the profiling results can reflect NeRF-based on-device 3D reconstruction bottlenecks for VR/AR devices. \ul{Profiling Method:} We follow a two-stage profiling: Stage~(1) characterizing the runtime of each step (or kernel to be more accurate) in the iNGP~\cite{muller2022instant} training process to locate the dominate steps and Stage~(2) profiling the DRAM bandwidth utilization and computation resource utilization of the dominant steps (and their corresponding back-propagation). The GPU runtime and resource utilization are measured from NVIDIA's \textit{nvprof}. \ul{Algorithm \& Datasets:} We evaluate iNGP~\cite{muller2022instant} on 8 datasets of Synthetic-NeRF~\cite{mildenhall2020nerf}. Each scene takes 3,500 iterations with a batch size of 256K samples per iteration.

\textbf{Profiling Results Analysis.} Although iNGP reduces the training time on the cloud GPU to a matter of seconds (i.e., 305.8s/scene as in Fig.~\ref{fig:iNGP_comp}(a)), the training on the edge GPUs, e.g., XNX and TX2, takes two/\todor{XX} hours per scene, respectively. We locate \textbf{four} efficiency-bottleneck steps/kernels from the training time breakdown in Fig.~\ref{fig:iNGP_comp}(b) (Since the training on XNX is \todor{XX}$\times$ faster than that on TX2, we only visualize XNX in Fig.~\ref{fig:iNGP_comp}): \textbf{Hashtable}, \textbf{Hashtable\_b}, \textbf{MLP$_{density}$}, and \textbf{MLP$_{color}$}. These steps/kernels (with their back-propagations) account for 76.4\% of the total training time. We profiled the DRAM read/write throughput and the FPU/ALU utilization as the achieved FPU (FP32 and FP16) and ALU (INT32) GFLOPs over the maximum GFLOPs provided by GPU of bottleneck steps/kernels in Fig.~\ref{fig:iNGP_kernel}. 

Based on profiling results, we have the following observations: \textbf{First}, we observe that these steps/kernels exhibit DRAM bandwidth-bound performance bottleneck, where the measured DRAM memory bandwidth utilization is 5.24$\sim$21.44$\times$ higher than FPU/ALU utilization. In particular, Hashtable/MLP$_{density}$/MLP$_{density}$\_b/MLP$_{color}$/ MLP$_{color}$\_b achieves 61.3\%/47.5\%/73.7\%/47.5\%/73.7\% DRAM bandwidth utilization (given the 59.7GB/s DRAM bandwidth) and $\leq$1.5\% FP32, $\leq$1.6\% FP16, $\leq$6.4\% INT32 utilization. We also note that the DRAM bandwidth and FPU/ALU utilization are both relatively low for Hashtable\_b, which results from that Hashtable\_b involves frequent write operations to update the feature vector's gradients and GPU schedules for grouping the write operations to the same gradient and cannot achieve ideal performance. \textbf{Second}, the underlying reasons for this memory-bound inefficiency are that (1) Random lookups to the hash table, which stores multi-level grids' feature vectors, require a high memory bandwidth and (2) The on-chip GPU cache capacity is too small for individual levels of the multiresolution hash table and intermediate data when processing MLPs. Specifically, an individual level of the hash table is 2MB which is 2$\sim$4$\times$ larger than available edge GPU cache capacity, let alone the 64MB intermediate data for MLP processing. \textbf{Third}, we find that index calculation, which is an important part for hash table lookups, consumes a large portion of total INT32 ALU utilization. For the current profiling, index calculation and GPU scheduling use INT32 data type and other algorithm-related computation uses FP32/FP16. We observe that INT32 ALU utilization is 4.2$\sim$160.7$\times$ higher than FP32/FP16 utilization. This motivates us to enable architecture support for index calculation in {\name}.

\subsection{Opportunity for NMP-based NeRF Training}
Offloading the memory-bound bottleneck steps to NMP architecture is a promising solution to boost NeRF training efficiency. Near-bank NMP architecture benefits from the 10$\times$ peak bandwidth improvement to solve the memory bandwidth bottleneck. In addition, the hundreds of MB memory per bank (i.e,. 256MB in our evaluation) provides enough memory capacity for steps in NeRF training. 



==> sections/backup_4-Algorithm.tex <==
\section{{\name} Algorithm \todor{Not Ready}}
\label{sec:alg}

Despite the memory bandwidth and memory capacity granted by near-bank NMP architecture, we need to tackle the challenges brought out by NMP 

\subsection{Locality-sensitive 3D Hashing Function}
\label{sec:hashing}

%%%%%%%%%%%%%% Begin of Figure %%%%%%%%%%%% 
\begin{figure}[b]
  \centering
  \includegraphics[width=0.1\linewidth]{figures/fig6_hashing.pdf}
\vspace{-1.em}
\caption{An illustration of mortron }
\vspace{-1.em}
\label{fig:alg_hashing}
\end{figure}
%%%%%%%%%%%%%%  End of Figure  %%%%%%%%%%%%

By leveraging the fact that 8 vertices of a 3D surrounding cube are always fetched together, we adopt a locality-sensitive 3D location hashing function to map the vertices close in the 3D scene to close hash table entries to overcome the reduced effective memory bandwidth challenge. The spatial hash function in iNGP~\cite{muller2022instant} show in Eq.~(\ref{eq:org_hash}) which will leads to the close coordinate points but far from in the hash table.
% \vspace{-1em}
\begin{align}
% h(\mathbf{x})=\left(\bigoplus_{i=1}^{3} x_{i} \pi_{i}\right) \quad \bmod T \label{eq:org_hash}
h(\mathbf{x}) &= (\pi_0x_0 \oplus \pi_1x_1 \oplus \pi_2x_2) \textrm{ mod } T, \label{eq:org_hash}
\end{align}
% \vspace{-1em}
where \(\oplus\) denotes the bit-wise \(\mathrm{XOR}\) operation, $x_{i}$ is per-dimension of input coordinate scaled by that level’s grid resolution, \(\pi_{i}\) are unique, large prime numbers and $T$ is the hash table size for each level~\cite{muller2022instant}.


To solve this, we replace the original hash encoding with morton encoding Eq.~(\ref{eq:zorder_hash}) knows as Z-order~\cite{z-order} which maps the 3D coordinate input to the hash table while preserving locality of the input points.
\begin{align}
f(\mathbf{x})=\left(x^{\prime}_{1} \oplus (x^{\prime}_{2} \ll 1) \oplus (x^{\prime}_{3} \ll 2) \right) \quad \bmod T \label{eq:zorder_hash}
\end{align}
where \(\oplus\) denotes the bit-wise \(\mathrm{XOR}\) operation and $x^{\prime}$ is the 32 bits binary format of each dimension through the Eq.~(\ref{eq:bit_expand}).
\begin{align}
x^{\prime}_{n+1}= (x^{\prime}_{n} * p_{n}) \land  q_{n}  \label{eq:bit_expand} \quad n=1,2,3,4
\end{align}
here, the binary format output $x^{\prime}$=$x^{\prime}_{4}$ and initial input is $x^{\prime}_{1}$=$x$. $p=\{$0x00010001, 0x00000101, 0x00000011, 0x00000005\} and $q=\{$0xFF0000FF, 0x0F00F00F, 0xC30C30C3, 0x49249249\}.

\subsection{Ray-first Point Stream Order}
\label{sec:point_stream_order}

%%%%%%%%%%%%%% Begin of Figure %%%%%%%%%%%% 
\begin{figure}[t]
  \centering
  \includegraphics[width=0.1\linewidth]{figures/fig6_hashing.pdf}
\vspace{-1.em}
\caption{An illustration of ray-first point stream order }
\vspace{-1.em}
\label{fig:alg_stream}
\end{figure}
%%%%%%%%%%%%%%  End of Figure  %%%%%%%%%%%%

Based on the fact that close points having the same surrounding cube will lookup the same hash table entries, we follow a ray-first point stream order to stream the close points sequentially for increased local register hit rates and reduced unnecessary memory requests.


==> sections/backup_4-Architecture.tex <==

% %%%%%%%%%%%%%% Begin of Figure %%%%%%%%%%%% 
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/fig9_fig10_temp.png}
% \vspace{-2.em}
% \caption{An exampled illustration of HT/MLP/MLP\_b/HT\_b when using \textit{parameter parallelism} and \textit{data parallelism} for HT/HT\_b and MLP/MLP\_b, respectively.}
% \vspace{-1.em}
% \label{fig:inter-bank}
% \end{figure*}
% %%%%%%%%%%%%%%  End of Figure  %%%%%%%%%%%% 

\section{{\name} Accelerator \todor{Not Ready}}
\label{sec:arch}

The {\name} architecture is deployed at one or several DRAM dies, where we integrate the {\name} microarchitecture near every memory bank (see Fig.~\ref{fig:lpddr}) to enjoy the bandwidth improvement. We call such a memory die as an {\name} accelerator. In this section, we first introduce the {\name} microarchitecture. Then, we present the hash table mapping scheme, which orchestrates the proposed algorithm-level techniques with {\name}'s near-bank NMP architecture. Finally, we discuss the inter-bank parallelism designs optimized for the involved steps/kernels.  

\subsection{{\name} Microarchitecture}
\label{sec:arch_overview}
As shown in Fig.~\ref{fig:hw_overall}, our {\name} microarchitecture mainly incorporates a computation engine and a controller. To read memory data into the computation engine, write data to the memory bank, or load instructions into the controller, our {\name} logic utilizes a commonly used structure where a data transfer MUX is directly connected to the bank's global row buffer via a row-buffer sized vector register (r0)~\cite{devic2022pim}. \ul{Computation Engine:} This engine is responsible for the computations of the offloaded bottleneck steps/kernels, which consists of two vector processing elements (PEs), three vector registers (r1, r2, and r3), a crossbar, as well as hash registers for hashing related hyper parameters (see Sec.~\ref{sec:alg_hash}). The two row-buffer sized vector PEs are for INT32 and FP32 arithmetic, respectively, to support index calculations and other algorithm-related computations. In addition, since NeRF training's bottleneck steps/kernels involve vector and matrix computations (e.g., trilinear interpolation and MLP), the PEs can adopt optimal dataflows to explore the reuse opportunities across vector/matrix. To support the PEs, the three vector registers feed input data to the PEs throughput the crossbar or store output data from PEs. PEs can directly read data from hash registers for hashing computations as well. \ul{Controller:} The controller has two main functionalities: controlling the processing of the computation engine and generating memory bank read/write commands and address. It is made of an instruction buffer, an instruction decoder, an address buffer, 



% After offloading bottleneck steps on the {\name} accelerator, the banks does not respond to the host processor until 


%%%%%%%%%%%%%% Begin of Figure %%%%%%%%%%%% 
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/fig6_arch.pdf}
\vspace{-1.em}
\caption{{\name} microarchitecture}
\vspace{-1.em}
\label{fig:hw_overall}
\end{figure}
%%%%%%%%%%%%%%  End of Figure  %%%%%%%%%%%% 


\subsection{Hash Table Mapping Scheme}
\label{sec:arch_datamapping}

\todob{91.7\%}
As the subarray parallelism makes the different subarrays in a bank to be accesses mostly independently, we further distribute the hash table to subarrays. 

%%%%%%%%%%%%%% Begin of Figure %%%%%%%%%%%% 
\begin{figure}[b]
  \centering
  \includegraphics[width=0.6\linewidth]{figures/download.png}
\vspace{-1.em}
\caption{Address distribution.  }
\vspace{-1.em}
\label{fig:hw_distribution}
\end{figure}
%%%%%%%%%%%%%%  End of Figure  %%%%%%%%%%%% 

\subsection{Inter-Bank Parallelism}
\label{sec:arch_parall}

It is natural to utilize inter-bank parallelism to distribute computations across memory banks to boost the NeRF training throughput. There are two approaches for inter-bank parallelism: \textit{data parallelism}, where each memory bank duplicates the parameters and processes different input data in parallel; and \textit{parameter parallelism} where each bank keeps part of the parameters and performs a part of computations based on the same input duplicated across banks. As limited by the I/O interface and the internal prefetch width (see Fig.~\ref{fig:lpddr}), the memory latency to access data in other banks is much higher than that in the local bank. Therefore, \textbf{minimizing the data movement amounts across different banks} is critical for an optimal inter-bank parallelism design. We classify the causes of inter-bank data movements as \ul{4 categories}: \ding{172}~the parameter/data duplication due to parallelism approaches, \ding{173}~the input/output data transfer between sequential steps/kernels, \ding{174}~the intermediate data transfer in a single step/kernel, and \ding{175}~the parameter gradient partial sum summation. Tab.~\ref{tab:data_size} illustrates the parameter and data sizes of the involved steps/kernels. Driven by these different memory patterns, we elaborate a \textbf{heterogeneous inter-bank parallelism} design to minimize the overall inter-bank data movements as follows: \textit{parameter parallelism} for $\text{HT}$/$\text{HT}_{\_\mathbf{b}}$ (i.e., level-by-level distributing the $L$-level multiresolution hash table to multiple banks) while \textit{data parallelism} for $\text{MLP}$/$\text{MLP}_{\_\mathbf{b}}$ (denoting the sequential $\text{MLP}_{\mathbf{d}}$$\rightarrow$$\text{MLP}_{\mathbf{c}}$ as MLP).

\textbf{Proposed Inter-bank Parallelism Analysis.} Fig.~\ref{fig:inter-bank} exemplifies the bottleneck steps run on an {\name} accelerator after adopting the proposed inter-bank parallelism design. We use Fig.~\ref{fig:inter-bank} to show how the design minimizes the 4 categories of inter-bank data movements. The parameter/data duplication amounts (Cat.\ding{172}) are minimized, since the much smaller parameter/input data, i.e., input data in $\text{HT}$ and parameters in $\text{MLP}$ (the sizes in Tab.~\ref{tab:data_size}), are duplicated. In addition, we only need one set of data transferred between sequential steps (Cat.\ding{173}), e.g., the output date of $\text{HT}$ which is the input data of MLP. Therefore, the inter-bank movements incurred Cat.\ding{173} are minimized as well. There is no intermediate data (Cat.\ding{174}) as shown in Fig.~\ref{fig:inter-bank}. Finally, the parameter gradient partial sum summation (Cat.\ding{175}) is constrained to the small MLPs to reduce the inter-bank gradient movements. 




%%%%%%%%%%%%%%  Begin of Table  %%%%%%%%%%%%
\begin{table}[t]
% \caption{Parameter/data sizes for the bottleneck steps/kernels in NeRF training.} 
\caption{Parameter/data sizes for the steps/kernels.} 
\begin{threeparttable}
\vspace{-0.8em}
\centering
%  \vspace{-1em}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\textbf{Steps/Kernels}} & \multirow{2}{*}{\textbf{Param.}$^{\triangleleft}$} & \textbf{Input} & \textbf{Output} & \textbf{Intermediate} \\ 
    &                & \textbf{Data$^{\diamond}$} & \textbf{Data$^{\diamond}$} & \textbf{Data$^{{\diamond},{\dagger}}$} \\ \hline
    $\text{HT}$      & 25MB    & 3MB   & 16MB  & 0 \\ \hline
    $\text{MLP}$$^*$        & 0.014MB & 16MB  & 1.5MB & 32MB \\ \hline
    $\text{MLP}_{\_\mathbf{b}}$$^*$     & 0.014MB & 1.5MB & 16MB  & 32MB \\ \hline
    $\text{HT}_{\_\mathbf{b}}$   & 25MB    & 16MB  & 0     & 0 \\ 
    % MLP/MLP\_b$^e$             & 0.014MB & 16MB & 1.5MB & 32MB \\ 
    % MLP$_{d}$/MLP$_{d}$\_b & 0.014MB & 16MB & 1.5MB & 32MB \\ \hline
    % MLP$_{c}$/MLP$_{c}$\_b & 0.014MB & 16MB & 1.5MB & 32MB \\
    \hline
\end{tabular}
}
\end{threeparttable}
\begin{tablenotes}
\footnotesize
\item{$^*$: $\text{MLP}$ stands for applying $\text{MLP}_{\mathbf{d}}$ and $\text{MLP}_{\mathbf{c}}$ sequentially.}
\item{$^{\triangleleft}$: The multiresolution hash table size and the two MLPs' weight size for HT/HT\_b and $\text{MLP}$/$\text{MLP}_{\_\mathbf{b}}$, respectively.}
\item{$^{\diamond}$: For a batch size of 256K sampled points.}
\item{$^{\dagger}$: The max intermediate data when doing level-by-level hash table lookup or layer-by-layer $\text{MLP}$ processing.}
\end{tablenotes}
\label{tab:data_size}
% \vspace{-1em}
\end{table} 
%%%%%%%%%%%%%%  End of Table    %%%%%%%%%%%%

%%%%%%%%%%%%%% Begin of Figure %%%%%%%%%%%% 
\begin{figure*}[b]
  \centering
  \includegraphics[width=1.05\linewidth]{figures/fig10_inter-bank_2.pdf}
\vspace{-1.em}
\caption{An exampled illustration of HT/MLP/MLP\_b/HT\_b when using \textit{parameter parallelism} and \textit{data parallelism} for HT/HT\_b and MLP/MLP\_b, respectively.}
\vspace{-1.em}
\label{fig:inter-bank}
\end{figure*}
%%%%%%%%%%%%%%  End of Figure  %%%%%%%%%%%% 



==> sections/backup_Related_Works.tex <==

\subsection{Near-Memory Processing}
\label{sec:NMP}


Processing-in-memory (PIM), which equips the memory system with the ability to perform computation, has been widely studied to solve the memory bound problems. One promising approach of PIM is near-memory processing (i.e., NMP) by adding or integrating the computation logics close to or inside the memory to take advantages of the larger internal bandwidth provided. For example, recent works deploy the computation logic at bank-level in DIMM to enjoy around 10$\times$ peak bandwidth improvement~\cite{devic2022pim}. The work~\cite{kim2012case} explores the subarray-parallelism to solve the bank conflicts. Prior studies exploit NMP architectures for general hashtable lookup~\cite{yitbarek2016exploring} and matrix-matrix multiplications in MLP workloads~\cite{shin2018mcdram}. Our {\name} distinguishes from the other works as we propose an algorithm-hardware co-design for NeRF's hashtable lookup and enable dedicated inter-bank parallelisms to support heterogeneous steps including MLPs. 
